Strategically revealing intentions in General Lotto games

Strategic decision-making in uncertain and adversarial environments is crucial for the security of modern systems and infrastructures. A salient feature of many optimal decision-making policies is a level of unpredictability, or randomness, which helps to keep an adversary uncertain about the system's behavior. This paper seeks to explore decision-making policies on the other end of the spectrum -- namely, whether there are benefits in revealing one's strategic intentions to an opponent before engaging in competition. We study these scenarios in a well-studied model of competitive resource allocation problem known as General Lotto games. In the classic formulation, two competing players simultaneously allocate their assets to a set of battlefields, and the resulting payoffs are derived in a zero-sum fashion. Here, we consider a multi-step extension where one of the players has the option to publicly pre-commit assets in a binding fashion to battlefields before play begins. In response, the opponent decides which of these battlefields to secure (or abandon) by matching the pre-commitment with its own assets. They then engage in a General Lotto game over the remaining set of battlefields. Interestingly, this paper highlights many scenarios where strategically revealing intentions can actually significantly improve one's payoff. This runs contrary to the conventional wisdom that randomness should be a central component of decision-making in adversarial environments.

==> preliminaries.tex <==
% !TEX root = main.tex

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%0000000000111111111122222222223333333333444444444455555555556666666666777777778
%2345678901234567890123456789012345678901234567890123456789012345678901234567890

Consider a two-player, constant-sum game consisting of two players, $A$ and $B$, simultaneously allocating their respective budgets, $X_A$ and $X_B$, over a set of $n\geq 2$ battlefields, $\mc{B}=\{1,\dots,n\}$.
Each battlefield $b\in\mc{B}$ has an associated value $v_b>0$, which is won by the player allocating more budget to $b$, i.e., given budget allocations $x_i=(x_{i,1},\dots,x_{i,n})\in\bb{R}^n$, $i=A,B$, the payoff to player $i$ is
\begin{equation}
    \sum_{b\in\mc{B}}\frac{v_b}{2}\cdot\left[1+{\rm sign}(x_{i,b}-x_{-i,b})\right],
\end{equation}
where $-i$ denotes the player opposing $i$.
For ease of notation, we assume player $A$ wins if there is a tie.

The \emph{Colonel Blotto game} is a game as defined above, where a valid budget allocation $x_i$ satisfies $x_{i,b}\geq 0$ for all $b\in\mc{B}$ and $\sum_{b\in\mc{B}}x_{i,b}\leq X_i$ for each player $i\in\{A,B\}$.
A valid mixed strategy in a Colonel Blotto game is an $n$-variate probability distribution function, $S_i: \mathbb{R}^n \to [0,1]$, with support only in the set of valid budget allocations.

The \emph{General Lotto game} is a variation on the Colonel Blotto game wherein a valid mixed strategy $S_i$ need only satisfy the budget constraint in expectation, i.e., for both $i \in \{A,B\}$,
\[  \sum^n_{b=1} \bb{E}_{S_{i,b}} [ x_{i,b} ] \leq X_i, \]
where $S_{i,b}:\bb{R} \to [0,1]$ is the univariate marginal distribution of $S_i$ corresponding to battlefield $b\in\mc{B}$.
% 
Note that the budget constraint is relaxed in the General Lotto game. Indeed, a budget allocation $\mathbf{x}_i$ such that $\sum^n_{b=1} x_b > X_i$ can still be attributed positive probability in the mixed strategy $S_i$ of a player $i \in \{A,B\}$.
%
Given player budgets $X_A, X_B > 0$, and a set of $n$ battlefields $\mc{B}$ {\color{red} with $\mathbf{v} = (v_1, \dots, v_n)$}, we denote the corresponding General Lotto game as ${\rm GL}(X_A,X_B,\mc{B})$. 

As both Colonel Blotto and General Lotto are constant-sum games, the players' equilibrium payoffs are unique. We reproduce the equilibrium payoffs of the General Lotto game here:
% 
\begin{fact}[General Lotto payoffs \cite{Kovenock_2012}]
    For player budgets $X_A, X_B > 0$, and $\phi = \sum_{b\in\mc{B}} v_b$, the equilibrium payoff to player $i \in \{A,B\}$ in the game ${\rm GL}(X_A,X_B,\mc{B})$ is $\phi \cdot L(X_i, X_{-i})$, where
    \begin{equation} \label{eq:twoplayer_payoff}
        L(X_i, X_{-i}) := 
        \begin{cases} 
            \frac{X_i}{2X_{-i}}& \quad \text{if } 0 < X_i \leq X_{-i} \\
            1 - \frac{X_{-i}}{2X_i}& \quad \text{if } X_i > X_{-i}.
        \end{cases} 
    \end{equation}
\end{fact}
When the number of battlefields is arbitrarily large, the players' equilibrium payoffs in the General Lotto game approximate those of the Colonel Blotto game arbitrarily closely (see \cite{Kovenock_2012} for a discussion) and are relatively simple to compute. 
For this reason, we consider the static General Lotto game as the primitive model of competitive resource allocation in the forthcoming multi-stage models.

